Word Sense Disambiguation as a Game of Neurosymbolic Darts

Word Sense Disambiguation (WSD) is one of the hardest tasks in natural language understanding and knowledge engineering. The glass ceiling of 80% F1 score is recently achieved through supervised deep-learning, enriched by a variety of knowledge graphs. Here, we propose a novel neurosymbolic methodology that is able to push the F1 score above 90%. The core of our methodology is a neurosymbolic sense embedding, in terms of a configuration of nested balls in n-dimensional space. The centre point of a ball well-preserves word embedding, which partially fix the locations of balls. Inclusion relations among balls precisely encode symbolic hypernym relations among senses, and enable simple logic deduction among sense embeddings, which cannot be realised before. We trained a Transformer to learn the mapping from a contextualized word embedding to its sense ball embedding, just like playing the game of darts (a game of shooting darts into a dartboard). A series of experiments are conducted by utilizing pre-training n-ball embeddings, which have the coverage of around 70% training data and 75% testing data in the benchmark WSD corpus. The F1 scores in experiments range from 90.1% to 100.0% in all six groups of test data-sets (each group has 4 testing data with different sizes of n-ball embeddings). Our novel neurosymbolic methodology has the potential to break the ceiling of deep-learning approaches for WSD. Limitations and extensions of our current works are listed.

==> review.tex <==

Purely data-driven supervised WSD approaches use feedforward networks \citep{hadiwinoto_navigli_2019} or transformers \citep{bevilacqua-navigli-2019-quasi} to  minimize a loss function $\mathcal{L}(w,c,s)$. In testing, the predicted sense is the one that maximizes the probability $P_{c,w,s}$, where $s$ is a possible of $w$ in the inventory. 
A popular baseline is the token tagger that can be described as follows: for each word $w$ in context $c$ produces a probability distribution $P_w$ over all senses. They feed pre-trained contextualized word embeddings into a feedforward network (Hadiwinoto 2019) or a transformer (Bevlacqua and Navigli 2019, Vial 2019), then multiply the output with a classification layer. 
The binary cross-entropy loss has been shown to be effective (Conia and Navigli, 2021), because it allows multiple annotations for a single instance that are available in the training set, rather than having to use a single ground-truth sense only. 
1-nn vector based approach (Peters 2018) creates sense embeddings by averaging the contextual vectors of instances within the training set. 
%\begin{eqnarray*}
%&&v^{c,w} = \mathrm{Embed}(c)_w\\
%&&v^{s}=\frac{1}{|\mathcal{D}^{(w,s)}|}\sum_{c'\in\mathcal{D}^{(w,s)}}\mathrm{Embed}(c')_w
%\end{eqnarray*}

\cite{Scarlini_aaai20} computed multilingual contextualized sense embeddings by utilizing BabeNet \citep{Navigli21BabelNet}, NASARI \citep{NASARI18}, and BERT \citep{devlin2018}. 


A generative variant of the sequence classification (Bevilacqua 2020) approaches the WSD problem as a natural language generation problem (NLG): given $c$ and $w$, the model should generate $\mathcal{G}(s)$. The approach has obtained results in the same ballpark of sequence classifiers, GlossBERT. This approach does not need for predefined sense inventories and is flexible to handle neologisms, compound words, slangs that are absent in standard WSD inventories. 


The utilising of relational knowledge within supervised learning introduces the joint learning of sense representation and the mapping from contextualized word embedding to sense classes \citep{blevins-zettlemoyer2020}.



The most popular English word-sense inventory is WordNet \citep{Miller90,MillerWordNet95} that consists of a large symbolic tree-liked  taxonomy of word-senses (some word-sense nodes in the taxonomy have more than two parent nodes, therefore, the taxonomy is not a pure tree structure). Each word sense has definitions ({\em glosses}) and sample usages. The largest word sense inventory is the BabelNet covering 500 languages and totalling 
over 20M synsets \citep{Navigli21BabelNet}. The largest manually annotated corpora is the SemCor \citep{semcor93} that has over 200,000 WordNet sense annotations. Annotation corpora can also be automatically developed using Web resources \citep{pasini2017,scarlini2019, Pasini2021}. 
    

Using glosses, WSD task can be tackled as a sequence classification problem (Huang 2019, Yap, 2020) $<w,c,\mathcal{G}(s)>$ and select the sense $\hat{s}$ with the highest score $$\hat{s}=argmax_{s'\in V^{(w)}}\Gamma(c,w,\mathcal{G}(s'))$$

ESCHER (Barba 2020) frames the WSD problem as a span extraction problem, given a target word in a sentence concatenated with all its possible definitions, a model has to find the span that best fits the target word use within the sentence. 





(For example, a PageRank-based algorithm can be developed to determine the probability of a given sense
being reached starting from the senses of its context words. Recent approaches of this kind have
been shown to obtain competitive results (Agirre
et al., 2014; Moro et al., 2014). However, due to
its inherent nature, knowledge-based WSD tends
to adopt bag-of-word approaches which do not exploit the local lexical context of a)


SyntagRank \citep{Navigli20kbdemo} is a purely graph-based approach that combines PageRank algorithm on WordNet augmented with WNG corpus and



\citep{KBWSD14,KBWSD18}
 SyntagNet \citep{maru_wsd19} that is a corpus with manually tagged relations between synsets.

SREF\_KB \citep{wang_wsd20} is a vector-based approach using contextualized word embeddings and sense embeddings. The sense vectors are computed by applying BERT on examples and definitions from WordNet. 

Pretrained language models are crucial in achieving high performance for both KG approaches and supervised WSD.  Pure KG approaches are completely outperformed the supervised approaches. The best SREF\_{KB} is 7.2\% better than the best supervised approach, ESCHER. 

Successful supervised methods are hybridized with KG methods.

Including knowledge is beneficial to WSD, as they are orthogonal to each other. 

The task of lexical substtution (McCarthy and Navigli, 2009) rquires the model to disambiguate a word in context by searching for meaning-preserving substitutes. 

Task of definition modeling (Noraset 2017) frames the dismabiguation task from NLU to NLG: instead of selecting the most relevant sense class, a system generates a description of its meaning. It is viewed as a promising way, as it expanding the scope of WSD without big sacrifices as a trade-off.

The WSD task is still not solved (Navigli 2018, Blevins, 2021). Current benchmarks are really starting to show their inadequacy. 

 

Alternative approaches like the generative lexicon , which provides a general framework
in which word meaning can be produced online, have been
proposed in the past, but no large-scale experiments have yet
been carried out on them.

A system’s performance, however, depends on the quality of the input representations. Furthermore, the inclusion of semantic features, in addition to lexical ones, has been proven effective in
many NLP approaches (Li and Jurafsky, 2015).

Word embeddings, the current paradigm for lexical representation of words, were popularized
with word2vec (Mikolov et al., 2013). The main
idea is to exploit a neural language model which
learns to predict a word occurrence given its surroundings. Another well-known word embedding
model was presented by Pennington et al. (2014),
which shares the idea of word2vec, but with the
difference that it uses explicit latent representations obtained from statistical calculation on word
co-occurrences. However, all word embedding
models share a common issue: they cannot capture polysemy since they conflate the various word
senses into a single vector representation. Several efforts have been presented so far to deal with
this problem. SensEmbed (Iacobacci et al., 2015)
uses a knowledge-based disambiguation system to
build a sense-annotated corpus that, in its turn, is
used to train a vector space model for word senses
with word2vec. AutoExtend (Rothe and Schutze ¨ ,
2015), instead, is initialized with a set of pretrained word embeddings, and induces sense and
synset vectors in the same semantic space using
an autoencoder. The vectors are induced by constraining their representation given the assumption
that synsets are sums of their lexemes. CamachoCollados et al. (2015) presented NASARI, an approach that learns sense vectors by exploiting the
hyperlink structure of the English Wikipedia, linking their representations to the semantic network
of BabelNet (Navigli and Ponzetto, 2012). More
recent works, such as ELMo (Peters et al., 2018)
and BERT (Devlin et al., 2019), are based on language models learned using complex neural network architectures. The advantage of these models is that they can produce different representations of words according to the context in which
they appear.




\paragraph{Representation power}

(Since there is a not insignificant number of instances where multiple similar senses of the target
word w fit the given context c (see Section 1), we
frame WSD as a multi-label classification problem
in which a machine learning model is trained to
predict whether a sense s $\in$ Sw is appropriate for a
word w in a given context c, independently of the
other senses in Sw. This is simply equivalent to
minimizing the binary cross-entropy loss)


It is assumed senses as opaque classes, which is valid in the pure neural computing, but not in the neurosymbolic setting
